Dynamic Choreographies - Safe Runtime Updates of Distributed Applications

Programming distributed applications free from communication deadlocks and races is complex. Preserving these properties when applications are updated at runtime is even harder. We present DIOC, a language for programming distributed applications that are free from deadlocks and races by construction. A DIOC program describes a whole distributed application as a unique entity (choreography). DIOC allows the programmer to specify which parts of the application can be updated. At runtime, these parts may be replaced by new DIOC fragments from outside the application. DIOC programs are compiled, generating code for each site, in a lower-level language called DPOC. We formalise both DIOC and DPOC semantics as labelled transition systems and prove the correctness of the compilation as a trace equivalence result. As corollaries, DPOC applications are free from communication deadlocks and races, even in presence of runtime updates.

==> projection.tex <==
\section{From AIOCs to APOCs}\label{sec:proj}

In this section we define the projection function to derive an APOC
network $\net$ implementing a given AIOC process ${\mathcal I}$ and an
initial global state $\Sigma$. To this end we first define an
auxiliary function $\pi:\mathit{AIOC \, processes} \times
\mathit{Roles} \rightarrow \mathit{APOC \,processes}$ that projects an
AIOC process on a given role. Before projecting, we find it convenient
to add unique keys identifying scopes, conditionals and cycles.  We
rely on keys, and we define \emph{annotated} AIOCs as AIOCs where
scopes, conditionals and cycles are annotated by unique keys as
follows:
\begin{itemize}
\item $\pscope{k}{l}{r}{\mathcal{I}}{\Delta}$
\item $\ifthenKey{e@r}{\mathcal{I}}{\mathcal{I}'}{k}$
\item $\whileKey{e@r}{\mathcal{I}}{k}$
\end{itemize}

Given an annotated AIOC process $\mathcal{I}$ and a role $s$, function
$\pi(\mathcal{I},s)$ is defined by structural induction on ${\mathcal
 % I}$ in Table~\ref{table:pi}.

\begin{table}[t!]
{
\footnotesize
\begin{tabular}{lll}
$
\pi(\comm{o^?}{r_1}{e}{r_1}{x} ,s)  =
\left \{ 
\begin{array}{ll}
\cout{o^?}{e}{r_2} & \mbox{ if } s=r_1\\
\cinp{o^?}{x}{r_1} & \mbox{ if } s= r_2\\
\one & \mbox{ otherwise}\\
\end{array}
\right.
$\\
$\pi(\one,s) = \one$\\
$\pi(\zero,s) = \zero$ \\
$\pi({\mathcal I};{\mathcal I}',s) = \pi({\mathcal I},s);\pi({\mathcal I}',s)$ 
\\
$\pi({\mathcal I} \parallel {\mathcal I}',s) = \pi({\mathcal I},s) \mid \pi({\mathcal I}',s)$
\\
$\pi(x@r = e,s) = 
\left \{ 
\begin{array}{ll}
x = e & \mbox{ if } s=r\\
\one & \mbox{ otherwise}\\
\end{array}
\right.
$\\
$ $\\
$
\pi(\ifthenKey{e@r}{\mathcal{I}}{\mathcal{I}'}{k},s) =$\\ 
$
\left \{ 
\begin{array}{ll}
\mbox{when } s=r:\\
k : \textsl{if} \; e \; \{ \prod_{r' \in \roles(\mathcal{I}) \cup \roles(\mathcal{I}')} \cout{o^*_k}{\mathit{true}}{r'} ; \pi(\mathcal{I},s)\}  \\
\textsl{else} \;  \{\prod_{r' \in \roles(\mathcal{I}) \cup \roles(\mathcal{I}')} \cout{o^*_k}{\mathit{false}}{r'}; 
\pi(\mathcal{I}',s)\}\\[1mm]
\mbox{when } s  \in \roles(\mathcal{I})\cup\roles(\mathcal{I}') \smallsetminus \{r\}:\\
\cinp{o^*_\ttk}{x_k}{r}; \ifthenKey{x_k}{\pi(\mathcal{I},s)}{\pi(\mathcal{I}',s)}{k}\\[1mm]
\mbox{otherwise}: \;\; \one\\
\end{array}
\right.
$\\
$ $\\
$\pi(\whileKey{e@r}{\mathcal{I}}{k},s) =$\\ 
$
\left \{ 
\begin{array}{l}
\mbox{when s = r}:\\
k: \textsl{while} \; e \; \{\prod_{r' \in \roles(\mathcal{I})} \cout{o^*_k}{\mathit{true}}{r'};\pi(\mathcal{I},s);\\
\qquad \prod_{r' \in \roles(\mathcal{I})} \cinp{o^*_k}{\_}{r'}\} ;
 \prod_{r'\in \roles(\mathcal{I})} \cout{o^*_k}{\mathit{false}}{r'}\\[1mm]
\mbox{when } s \in\roles(\mathcal{I}) \smallsetminus \{r\}:\\
\cinp{o^*}{x_k}{r}; \while{x_k}{\pi(\mathcal{I},s); \cout{o^*_k}{\texttt{ok}}{r};\cinp{o^*_k}{x_k}{r}}\\[1mm]
\mbox{otherwise}: \one
\end{array}
\right.
$\\
$ $\\
$
\pi(k: \scope{l}{r}{\mathcal I}{\Delta}{A},s) =$\\ 
$
\left \{ 
\begin{array}{l}
\mbox{when } s = r:\\
\pscope{k}{l}{r}{\pi({\mathcal I},s)}{\Delta}{\roles({\mathcal I})}\\[1mm]
\mbox{when } s \in \roles(\mathcal{I}) \smallsetminus \{r\}:\\
\psscope{k}{l}{r}{\pi({\mathcal I},s)}\\[1mm]
 \mbox{otherwise}: \one\\
\end{array}
\right.
$
\end{tabular}}
\caption{Process-projection function $\pi$}\label{table:pi}
\end{table}

Function $\pi$ is used to derive an APOC process from an AIOC. It is
used both to derive the starting APOC processes from a given AIOC, and
to apply an adaptation rule to a running APOC system (cfr.\ rule {\sc
  Lead-Adapt} in Table~\ref{table:pocasynchlts}). 

Here we use function $\pi$ to define function $\proj: \mathit{AIOC \ processes} \times \mathit{States} \rightarrow \mathit{APOC \ network}$ that, given an AIOC process $\mathcal{I}$ and a global state $\Sigma$, returns the APOC network $\proj(\mathcal{I}, \Sigma)$. 
%
We denote with $\parallel_{i \in I} \net_i$ the parallel composition of networks $\net_i$ for each $i \in I$.
%
\begin{definition}[Projection]
The projection of an AIOC process ${\mathcal I}$ with initial global state $\Sigma$ is the APOC network defined by:
$$\proj({\mathcal I},\Sigma)=\parallel_{s \in \roles({\mathcal I})} \role{\pi({\mathcal I},s), 
\Sigma_s}{s}$$
\end{definition}
%

